GraphAGILE: An FPGA-based Overlay Accelerator for Low-latency GNN Inference

This paper presents GraphAGILE, a domain-specific FPGA-based overlay accelerator for graph neural network (GNN) inference. GraphAGILE consists of (1) \emph{a novel unified architecture design} with an \emph{instruction set}, and (2) \emph{a compiler} built upon the instruction set that can quickly generate optimized code. Due to the proposed instruction set architecture (ISA) and the compiler, GraphAGILE does not require any FPGA reconfiguration when performing inference on various GNN models and input graphs. For the architecture design, we propose a novel hardware module named Adaptive Computation Kernel (ACK), that can execute various computation kernels of GNNs, including general matrix multiplication (GEMM), sparse-dense matrix multiplication (SpDMM) and sampled dense-dense matrix multiplication (SDDMM). The compiler takes the specifications of a GNN model and the graph meta data (e.g., the number of vertices and edges) as input, and generates a sequence of instructions for inference execution. We develop the following compiler optimizations to reduce inference latency: (1) computation order optimization that automatically reorders the computation graph to reduce the total computation complexity, (2) layer fusion that merges adjacent layers to reduce data communication volume, (3) data partitioning with a partition-centric execution scheme that partitions the input graph to fit the available on-chip memory of FPGA, (4) kernel mapping that automatically selects execution mode for ACK, and performs task scheduling to overlap computation with data communication and achieves dynamic load balance. We implement GraphAGILE on a state-of-the-art FPGA platform, Xilinx Alveo U250. GraphAGILE can execute widely used GNN models, including GCN, GAT, GIN, GraphSAGE, SGC and other GNN models supported by GraphGym.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> appendex.tex <==
\appendices

% \begin{figure*}[h]
%      \centering
%      \includegraphics[width=17cm]{picAppendix/instruction-set.pdf}
%      \caption{GraphAGILE high-level instruction fields}
%      \label{app:fig:instruction-sets}
% \end{figure*}


\section{Details of the instruction set}
\label{app:sub:instruction-set}

\subsection{High-level Instructions}
% All the high-level instructions have the uniform 128-bit length and the instruction fields are depicted in Figure \ref{app:fig:instruction-sets}. The $\verb|OPCODE|$ field indicates the type of instruction. Other fields contain the instruction-specific information. 
% \begin{itemize}
%     \item \emph{Control and Scheduling Instructions (CSI)}: A CSI defines the computation workload of a layer block (See Algorithms \ref{algo:PCFA}, \ref{algo:Vector-Inn}, \ref{algo:Vector-Add}). $\verb|num_of_tiling_block|$ indicates the number of tiling blocks in the current layer block. Thereby, the scheduler assigns the tiling blocks of the current layer to the PEs (See Algorithm \ref{algo:task-scheduling}).
%     \item \emph{Memory Read/Write Instructions}: A memory read/{\color{red}write} instruction loads/stores the data  (model weights, edges, vertex feature vectors) from/to the FPGA local DDR memory. $\verb|sram_ID|$ indicates the on-chip buffer ID. $\verb|SRAM_BASE|$ indicates the base address of the on-chip buffer.  $\verb|DRAM_BASE|$ indicates the base address of FPGA DDR. $\verb|INFO|$ contains the information of current memory transaction, such as transaction length,  etc.
%     \item \emph{GEMM Instructions}: A GEMM instruction contains the information of the matrix multiplication between a large block weight matrix (in the Weight Buffer) and a large block of feature matrix (in the Feature Buffer). Due to the double buffering technique, we use $\verb|Feature Buffer ID|$ and $\verb|Weight Buffer ID|$ to indicate which buffer to use.
%     \item \emph{SpDMM Instructions}: A SpDMM instruction defines  multiplication of a  block of sparse adjacency matrix with a block of dense feature matrix. See Section \ref{subsec:data-partitioing} for the details of data tiling. The block of adjacency matrix  is stored in the Edge Buffer specified by $\verb|Edge Buffer ID|$. The block of dense feature matrix  is stored in Feature Buffer specified by $\verb|Feature Buffer ID|$. $\verb|num_edge|$ indicates the number of edges in the sparse adjacency matrix.
%     \item \emph{SDDMM Instructions}: Similar to a SpDMM kernel, a SDDMM kernel involves the operations between a block of sparse adjacency matrix and a block of {\color{red}dense} feature matrix (See Algorithm \ref{algo:Vector-Inn}). Therefore, a SDDMM instruction has similar fields as a SpDMM instruction.
%     \item \emph{Preprocessing/Post Processing  Instructions}: a preprocessing instruction initializes the data in a buffer and the Post Processing Instruction performs element-wise activation function for a buffer. $\verb|sram_ID|$ indicates which buffer to process. 
% \end{itemize}

\subsection{Microcode}
In a PE of GraphAGILE, the Instruction Decoder \& Control Signal Generator reads high-level instructions from Instruction Queue. Then, each high-level instruction is translated to a sequence of microcode to execute the tasks defined in the high-level instruction. The microcode of each high-level instruction is stored in Microcode Table and the code translation is performed by looking up the Microcode Table at runtime.


% \noindent \textbf{Microcode of GEMM instructions}:
% \begin{figure}[h]
%      \centering
%      \vspace{-0.3cm}
%      \includegraphics[width=7cm]{pic/GEMM-microcodepdf.pdf}
%      \vspace{-0.2cm}
%      \caption{GEMM between a block of feature matrix $\bm{H}_{B}$ (stored in Feature Buffer) and a block of weight matrix $\bm{W}_{B}$ (stored in Weight Buffer)}
%      \label{fig:structure-ALU}
% \end{figure}
% A high-level GEMM instruction is translated to a sequence of microcode to execute the GEMM between a block of feature matrix $\bm{H}_{B}\in \mathbb{R}^{S_{B}\times Len}$ and a block of weight matrix $\bm{W}_{B} \in \mathbb{R}^{Len \times G_{B}}$. The Pseudocode of the sequence of microcode is described in Algorithm \ref{algo:Pseudocode-of-GEMM-instruction}. In GEMM mode, the Adaptive Computation Kernel (ACK) works as 2-D systolic array of size $p_{\text{sys}} \times p_{\text{sys}}$ using output-stationary dataflow. In each clock cycle, ACK receives  $p_{\text{sys}}$ data from Feature Buffer and $p_{\text{sys}}$ data from Weight Buffer, respectively. In Feature Buffer, $\bm{H}_{B}$ is further partitioned to small data tiles along row dimensions and each data tile $\bm{H}_{T:i}$ has $p_{\text{sys}}$ rows. Similarly, in Weight Buffer, $\bm{W}_{B}$ is partitioned to small data tiles along {\color{red}column} dimension and each data tile $\bm{W}_{T:i}$ has $p_{\text{sys}}$ columns of $\bm{W}_{B}$. $\bm{H}_{\text{out}:ij}$ denotes the result of the multiplication between $\bm{H}_{T:i}$ and $\bm{W}_{T:j}$.


 
 
% \begin{algorithm}
%  \caption{Pseudocode of GEMM microcode}
%  \begin{algorithmic}[1]
%  \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
%  \Require $\bm{H}_{B}$; $\bm{W}_{B}$
%  \Ensure $\bm{H}_{\text{out}}$
% \For{$i \leftarrow 1$ to $\frac{S_{B}}{p_{\text{sys}}}$}
%     \For{$j \leftarrow 1$ to $\frac{G_{B}}{p_{\text{sys}}}$}
%         \State // {\color{blue}Pipelined execution of $\bm{H}_{\text{out}:ij} = \bm{H}_{T:i} \times \bm{W}_{T:j}$}
%         \For{$k \leftarrow 1$ to $Len$ \textbf{Parallel}}
%             \State Load the $p_{sys}$ data of $k^{\text{th}}$ column of $\bm{H}_{T:i}$ \hspace*{5em}  and send them to ACK
%             \State Load the $p_{sys}$ data of  $k^{\text{th}}$ row of $\bm{W}_{T:j}$  and  \hspace*{5em}  send them to ACK
%         \EndFor
%     \EndFor
% \EndFor
%   \end{algorithmic} 
%  \label{algo:Pseudocode-of-GEMM-instruction}
%  \end{algorithm}


% \begin{algorithm}
%  \caption{Pseudocode of SpDMM microcode}
%  \begin{algorithmic}[1]
%  \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
%  \Require $\bm{H}_{B}$; $\bm{A}_{B}$; number of edges in $\bm{A}_{B}$: $N_{e}$
%  \Ensure $\bm{H}_{\text{out}}$
% \For{$i \leftarrow 1$ to $\frac{2N_{e}}{p_{\text{sys}}}$}  {\color{blue}\Comment{Pipelined execution of SpDMM}}
%     \State Load $\frac{p_{\text{sys}}}{2}$ unprocessed edges from $\bm{A}_{B}$ in Edge Buffer 
%     \State Send the $\frac{p_{\text{sys}}}{2}$ edges to Index Shuffle Network (ISN)
% \EndFor
%   \end{algorithmic} 
%  \label{algo:Pseudocode-of-SpDMM-instruction}
%  \end{algorithm}
 
% \vspace{0.1cm}
% \noindent \textbf{Microcode of SpDMM instructions}:
% A high-level SpDMM instruction is translated to a sequence of microcode to execute the SpDMM between a block of feature matrix $\bm{H}_{B}$ (stored in the Feature Buffer) and a block of sparse adjacency matrix $\bm{A}_{B}$ (stored in the Edge Buffer). The execution of SpDMM is edge-centric (See Section \ref{subsec:Adaptive-Computation-Kernel}). Therefore, in each clock cycle, $\frac{p_{\text{sys}}}{2}$ unprocessed edges in $\bm{A}_{B}$ are fetched from Edge Buffer. The $\frac{p_{\text{sys}}}{2}$ edges are sent to Index Shuffle Network to execute feature aggregation. 



% \begin{algorithm}
%  \caption{Pseudocode of SDDMM microcode}
%  \begin{algorithmic}[1]
%  \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
%  \Require $\bm{H}_{B}$; $\bm{A}_{B}$; number of edges in $\bm{A}_{B}$: $N_{e}$
%  \Ensure weights of all the edges in $\bm{A}_{B}$
% \For{$i \leftarrow 1$ to $\frac{2N_{e}}{p_{\text{sys}}}$} {\color{blue}\Comment{Pipelined execution of SDDMM}}
%     \State Load $\frac{p_{\text{sys}}}{2}$ unprocessed edges from $\bm{A}_{B}$ in Edge Buffer
%     \State Extract the $\frac{p_{\text{sys}}}{2}$ $src$ indices and $\frac{p_{\text{sys}}}{2}$ $dst$ indices
%     \State Send the $p_{\text{sys}}$ indices to ISN
% \EndFor
%   \end{algorithmic} 
%  \label{algo:Pseudocode-of-SDDMM-instruction}
%  \end{algorithm}
% \vspace{0.1cm}
% \noindent \textbf{Microcode of SDDMM instructions}:
% A high-level SDDMM instruction is translated to a sequence of microcode to execute the SDDMM using a block of feature matrix $\bm{H}_{B}$ (stored in the Feature Buffer) and a block of sparse adjacency matrix $\bm{A}_{B}$ (stored in the Edge Buffer). Similar to SpDMM, the execution of SDDMM is edge-centric (See Section \ref{subsec:Adaptive-Computation-Kernel}). In each clock cycle, $\frac{p_{\text{sys}}}{2}$ unprocessed edges in $\bm{A}_{B}$ are fetched from Edge Buffer. The $\frac{p_{\text{sys}}}{2}$ $src$ indices and $\frac{p_{\text{sys}}}{2}$ $dst$ indices  are extracted from the $\frac{p_{\text{sys}}}{2}$ unprocessed edges. Then, the total $p_{\text{sys}}$ indices are sent to Index Shuffle Network (ISN) to execute the SDDMM of $\bm{A}_{B}$ and $\bm{H}_{B}$. 


\subsection{Vector Addition Mode}
\label{app:Vector-Addition-Mode}
% In Vector Addition Mode, the basic operation is the addition of two feature vectors. An Update Unit (See Figure \ref{fig:arch-ack}) works as a vector adder. To add $\bm{h}_{\text{u}}$ and $\bm{h}_{\text{v}}$, the indices $u$ and $v$ are routed through Index Shuffle Network (ISN) to Feature Buffer to fetch $\bm{h}_{\text{u}}$ and $\bm{h}_{\text{v}}$. Then $\bm{h}_{\text{u}}$ and $\bm{h}_{\text{v}}$ are routed to an Update Unit through Data Shuffle Network (DSN) to perform vector addition. The results will bypass the Reduction Unit and are sent back to Feature Buffer.  The ACK can execute $p_{\text{sys}}/2$ vector additions of length $p_{\text{sys}}$ at  each clock cycle. Two feature vectors of length $|\bm{h}_{i}|$ can be added in $\lceil \frac{|\bm{h}_{i}|}{p_{\text{sys}}} \rceil$ cycles.

\section{Compiler Optimizations}
\label{app:Compiler-Optimization}

\subsection{Computation Order Optimization}
\label{app:Order-Optimization}


% We design the general rule for the  computation order optimization.  First, we define the  \emph{linear operator} in the aggregate layer:
% % in Theorem \ref{theorem:computation-order}. 
% \begin{definition}
% In an Aggregate layer, the aggregation operator $\text{AggOp}()$ is a linear operator if $\text{AggOp}()$ satisfies the following two properties:
% \begin{itemize}
%     \item $\text{AggOp}(\bm{h}_{x} + \bm{h}_{y}) = \text{AggOp}(\bm{h}_{x}) + \text{AggOp}(\bm{h}_{y})$ for any $\bm{h}_{x} \in \mathbb{R}^{f}$ and  $\bm{h}_{y} \in \mathbb{R}^{f}$.
%     \item $\text{AggOp}(c\bm{h}_{x}) = c\text{AggOp}(\bm{h}_{x})$ for any $\bm{h}_{x} \in \mathbb{R}^{f}$ and any constant $c$. 
% \end{itemize}
% \hspace{0.4cm} For example, Sum() is a linear operator while {\color{red}Max()} is a non-linear operator. 
% \end{definition}
% Then, we identify the  exchangeability of computation order in Theorem \ref{theorem:computation-order}:
% \begin{theorem}
% \label{theorem:computation-order}
% For a pair of adjacent Aggregate layer and Linear Layer, if the Aggregation operator $\text{AggOp}()$ of the Aggregate layer is a \emph{linear operator}, we can exchange the computation order of this Aggregate layer and Linear Layer.
% % A \emph{linear operator} $\text{AggOp}()$ has the two properties:
% \end{theorem} 
% \begin{proof*}
% The computation process of the adjacent Aggregate layer and Linear layer can be expressed as:
% \begin{equation}
%     \bm{h}_{i}^{l} = \text{AggOp}(\bm{A}_{j,i} \times \bm{h}_{j}^{l-1} \times \bm{W}, j \in \mathcal{N}(i))
% \end{equation}
% where AggOp() is the aggregation operator of the Aggregate layer and the $\bm{W}$ is the weight matrix of the Linear layer. Since the operator AggOp() is a linear operator, the above equation can be written as:
% \begin{equation}
%     \bm{h}_{i}^{l} = \text{AggOp}(\bm{A}_{j,i} \times \bm{h}_{j}^{l-1}, j \in \mathcal{N}(i))  \times \bm{W}
% \end{equation}
% Therefore, the computation order of this pair of Aggregate layer and Linear layer can be exchanged without affecting the final result. 
% \end{proof*}
% \vspace{0.2cm}
% The computation order can affect the total computation complexity. The computation complexity (CC) of an Aggregate layer is:
% \begin{equation}
%     \text{CC}_{\text{Aggregate}} (f_{\text{in}}, f_{\text{out}}, |\mathcal{E}|)= 2 \cdot f_{in} \cdot |\mathcal{E}|, (f_{\text{in}} = f_{\text{out}})
% \end{equation}
% The computation complexity (CC) of a Linear layer is:
% \begin{equation}
%     \text{CC}_{\text{Linear}} (f_{\text{in}}, f_{\text{out}}, |\mathcal{V}|)=  2 \cdot f_{\text{in}} \cdot f_{\text{out}} \cdot |\mathcal{V}|
% \end{equation}
% Suppose the feature vector to the Aggregate-Linear pair (An Aggregate layer followed by a Linear layer) has length $f_{1}$, the output feature vector has length $f_{2}$. The computation complexity of this Aggregate-Linear pair is:
% \begin{equation}
%   \text{CC}_{\text{Aggregate-Linear}} = 2 \cdot f_{1} \cdot \mathcal{|E|} +2 \cdot f_{1} \cdot f_{2} \cdot \mathcal{|V|} \label{eq:Aggregate-Linear-execution-order}
% \end{equation}
% If the Aggregate layer and the Linear layer is exchangeable, the computation complexity after the exchange is:
% \begin{equation}
%     \text{CC}_{\text{Linear-Aggregate}} =2 \cdot f_{1} \cdot f_{2} \cdot \mathcal{|V|} + 2 \cdot f_{2} \cdot \mathcal{|E|} \label{eq:Linear-Aggregate-execution-order}
% \end{equation}
% \begin{theorem}
% \label{theorem:computation-complexity}
% Based on Equation (\ref{eq:Aggregate-Linear-execution-order}) and (\ref{eq:Linear-Aggregate-execution-order}),  if $f_{1} >f_{2}$,  Linear-Aggregate execution order has lower complexity. If $f_{2} >f_{1}$ Aggregate-Linear execution order has lower complexity. 
% \end{theorem} 
% Based on Theorem \ref{theorem:computation-order} and Theorem \ref{theorem:computation-complexity}, we propose the computation order optimization as shown in Algorithm \ref{algo:computation-order-optimization} (Section \ref{subsec:Computation-Order-Optimization}).

\subsection{Data Partitioning}
\label{app:data-partitioning}

\vspace{0.1cm}


%  \tikzmark{start2}  \tikzmark{end2} 






% \vspace{0.1cm}
% \noindent \textbf{Small Graph}: For small graphs of which feature matrix and edges can be completely stored in the on-chip buffers,  the memory read instructions from/to external DDR memory is eliminated to reduce the inference latency. The first layer will keep the memory read instructions and the last layer will keep the memory write instructions.
 






\section{Implementation Details}
\label{app:Implementation-Details}

% \subsection{Arithmetic Logic Unit (ALU)}

% \begin{figure}[h]
%      \centering
%      \vspace{-0.3cm}
%      \includegraphics[width=7cm]{pic/ALU-ACT.pdf}
%      \vspace{-0.2cm}
%      \caption{The structure of the ALU in ACK and the structure of an Activation Element in Activation Unit}
%      \label{fig:structure-ALU}
% \end{figure}


% The proposed ALU can support multiplication, addition, multiply-add operation, comparison (Mux, Min), ReLU activation, PReLU activation. Each PE also has an Activation Unit and the Activation Unit has 16 Activation Elements (See Figure \ref{fig:structure-ALU}) that  work in parallel. The Activation Element supports exponential function $\verb|exp(x)|$, sigmoid function $\verb|1/(1+exp(x))|$, division. 

% \subsection{Routing Network}
% \label{app:Routing Network}

% \begin{figure}[h]
%      \centering
%      \includegraphics[width=8.5cm]{pic/butter-fly.pdf}
%      \vspace{-0.3cm}
%      \caption{The structure of ISN and DSN ($p_{\text{sys}} = 8$)}
%      \vspace{-0.3cm}
%      \label{fig:Bufferfly}
% \end{figure}

% The proposed Index Shuffle Network (ISN) and Data Shuffle Network (DSN) are implemented using Bufferfly Network that is proposed in \cite{choi2021hbm}. The structure of the Bufferfly Network is depicted in Figure \ref{fig:Bufferfly}. The benefits of using this Bufferfly Network are: (1) the Bufferfly Network is hardware efficient that only consume a small amount of ALUs, (2) there are intermediate buffers in the Switches that can buffer data when there is network congestion. As {\color{red}shown} in \cite{choi2021hbm}, such intermediate buffers lead to high-throughput data routing. 





% \subsection{RAW Unit}
% \label{app:RAW-Unit}

%  In SpDMM mode, read-after-write (RAW) data hazard may occur when accumulators in the Gather Unit read the old feature vertex vector from the Feature/Result Buffer.
%  To resolve the RAW data hazard, we implement a RAW Unit before Gather Unit as shown in Figure \ref{fig:RAWUnit-Arch}. In the RAW Unit, there is a RAW detector to detect the RAW data hazard and a small Reorder Buffer (implemented as a FIFO) to cache the input data when RAW is detected. The data in the Reorder Buffer will be sent to Gather Unit when there is no RAW data hazard.
 

% \begin{figure}[h]
%   \centering
%     \includegraphics[width=5cm]{pic/RAWUnit.pdf}
%     \captionof{figure}{RAW Unit}
%      \label{fig:RAWUnit-Arch}
% \end{figure}


% \begin{algorithm}
%  \caption{Partition-Centric  execution scheme of an Vector-Add Layer}
%  \begin{algorithmic}[1]
%  \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
%  \Require $\bm{H}_{\text{in}}^{l_{1}}$, $\bm{H}_{\text{in}}^{l_{2}}$
%  \Ensure $\bm{H}_{\text{out}}$
%  \State \tikzmark{start4} \emph{Execution of a Vector-Add layer}
% \For{$i\leftarrow 1$ to $\frac{f_{\text{in}}}{N_{2}}$ } 
%     \For{$j\leftarrow 1$ to $\frac{|V|}{N_{1}}$ } 
%         \If{there is an idle PE: $\text{PE}_{p}$}
%             % \State Assign $\bm{H}_{\text{out}}(i, j)$ to $\text{PE}_{i}$
%             \State Assign $\bm{H}_{\text{out}}(i, j)$ to $\text{PE}_{p}$
%             \State \tikzmark{start3}  \hspace{-0.2cm}   load  $\bm{H}_{\text{in}}^{l_{1}}(i, j)$ to Feature Buffer
%             \State load  $\bm{H}_{\text{in}}^{l_{2}}(i, j)$ to Feature Buffer

%             \State $\bm{H}_{\text{out}}(i, j) \leftarrow \text{VecAdd}(\bm{H}_{\text{in}}^{l_{1}}(i, j), \bm{H}_{\text{in}}^{l_{2}}(i, j))$
%             \State Store $\bm{H}_{\text{out}}(i, j)$  \tikzmark{end3} \tikzmark{end4}
%         \EndIf
%     \EndFor
% \EndFor
% \end{algorithmic} 
% \label{algo:Vector-Add}
% \end{algorithm}
%  \Textbox[4.4cm]{start3}{end3}{Tiling Block}
% \Textbox[4.3cm]{start4}{end4}{Layer Block}

% \subsection{System Details of Alveo U250}

% {\color{red}Figure \ref{fig:structure-ALU} depicts} the structure of an ALU in the ACK.   Each PE has an Index Shuffle Network and a Data Shuffle Network. The Index Shuffle Network has 16 input ports and 16 output ports. Each port has 96 bits since an edge is  96-bit (32-bit source index, 32-bit destination index, 32-bit edge weight).  The Data shuffle network also has 16 input ports and 16 output ports. Each port has $(16+3)\times32$ bits where $16 \times 32$ bits are used for vector features and $3 \times 32$ bits are used for edges. Both Index Shuffle Network and Data Shuffle Network are implemented using a butterfly network. Each PE has Edge Buffer of size 2MB, Feature Buffer of size 3MB, and Weight Buffer of size 1MB. We exploit double buffering technique for Edge Buffer and Weight Buffer, and triple buffering technique for Feature Buffer. Such triple/double buffering enables the overlapping of computation and data communication.  The dimension of a Weight Buffer is $(N_{W} = 16384)\times (P_{\text{sys}}=16)$, the dimension of an Edge Buffer is $(N_{E}=65K)\times 3$, the dimension of a Feature Buffer is $(N_{F1}=16384)\times (N_{F2}=16)$.




% \subsection{Resource utilization of various FPGA accelerators}
% \label{app:fpga-resource-utilization}

% Table \ref{tab:resource-utilizations} shows the resource utilization of various FPGA accelerators in the experiments.


% \begin{table}[!ht]
% \centering
% \caption{Specifications of FPGA accelerators in the experiments }
% \vspace{-0.2cm}
% \begin{threeparttable}
% \begin{adjustbox}{max width=0.48\textwidth}
% \begin{tabular}{c|ccc}
%  \toprule
%            %\\ \midrule
% \textbf{Platforms} &  AWB-GCN \cite{geng2020awb} &  BoostGCN \cite{zhang2021boostgcn} & GraphAGILE  \\ 
% \midrule \midrule 
% Platform  &  Stratix 10 SX &  Stratix 10 GX  & Alveo U250  \\
% %  { Platform Release Year}    &  2020 &  2020 &  & & &   2018 \\
%  {Platform Technology}  &  Intel 14 nm & Intel 14 nm &  TSMC 16 nm\\ 
% {Frequency} & 330 MHz  & 250 MHz & 300 MHz \\  
% LUTs/ALMs & 200K-300K ALMs & 294K ALMs & 778K LUTs \\
% DSPs & 4096 (Intel DSP) & 3840 (Intel DSP) & 10240 (Xilinx DSP) \\
% {Peak Performance}& 1351 GFLOPS & 640  GFLOPS & 614 GFLOPS  \\ 
% {On-chip Memory}& 22MB & 32 MB & 45 MB   \\
% {Memory Bandwidth}& 57.3 GB/s & 77 GB/s  & 77 GB/s \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{threeparttable}
% \label{tab:resource-utilizations}
% \end{table}

%  778K LUTs (45%), 10240 DSPs (83%), 1853 BRAMs (69%) and 1050 URAMs (82%
% \subsection{FPGA Resource Utilization}

% \section{Advantages of GraphAGILE}
% \label{app:advantages}


% \section{Load balance}
% \label{app:load-imbalance}

% The key benefit of GraphAGILE is that we use a single hardware module (ACK) to execute various computation kernels with high efficiency. Therefore, we are able to assign all the on-chip  computation resources to ACKs. In the hybrid accelerators (e.g., HyGCN \cite{yan2020hygcn}, BoostGCN \cite{zhang2021boostgcn}), the  computation resources are divided among different hardware modules to execute different computation kernels. 
% % Therefore, in hybrid accelerators, the load imbalance among the hardware modules can lead to hardware under-utilization.
% Suppose for a single GCN layer, feature aggregatgion (FA) has the workload $\alpha_{1}$ $(\alpha_{1} >0)$ and feature transformation (FT) has the workload $\alpha_{2}$ $(\alpha_{2} >0)$, and the total computation resource is $\beta$. In our design, we use $\beta$ for ACKs. Therefore, the latency for executing this single GCN layer of our design is: $\frac{\alpha_{1} + \alpha_{2}}{\beta}$. In the hybrid accelerator, suppose the hardware module for FA uses $\beta_{1}$ resources and the hardware module for FT uses $\beta - \beta_{1}$ resources. The latency for executing this single GCN layer is $\max \left(\frac{\alpha_{1}}{\beta_{1}} , \frac{\alpha_{2}}{\beta - \beta_{1}}\right)$. It can be proved that:
% \begin{equation}
%     \frac{\alpha_{1} + \alpha_{2}}{\beta} \leqslant \max \left(\frac{\alpha_{1}}{\beta_{1}}, \frac{\alpha_{2}}{\beta - \beta_{1}}\right) \quad(\beta > 0, \beta_{1} >0, \beta - \beta_{1} >0)
% \end{equation}
% $\frac{\alpha_{1} + \alpha_{2}}{\beta} = \max \left( \frac{\alpha_{1}}{\beta_{1}}, \frac{\alpha_{2}}{\beta - \beta_{1}}\right) $
% % {\color{blue}seems wrong?? $\frac{\alpha_1+\alpha_2}{\beta} = \frac{\alpha_1}{\beta}+\frac{\alpha_2}{\beta}<\frac{\alpha_1}{\beta_1}+\frac{\alpha_2}{\beta-\beta_1}$\color{black}}
% when $\frac{\alpha_{1}}{\beta_{1}}  = \frac{\alpha_{2}}{\beta - \beta_{1}}$.
% In the GNN model, the workload of FA $\alpha_{1}$ is usually unpredictable because the number of edges depends on the connectivity of the input graph.   Therefore, in a fixed hybrid accelerator, it is hard to keep load balance for various input graphs and variou GNN models. The load imbalance incurs increased latency. To execute GNN models with more than two computation kernels (e.g., GAT), load imbalance can be more severe in hybrid accelerators.


% \section{Fourth Appendix}
% \label{FourthAppendix}
  

==> ariv.tex <==
\begin{scriptsize}
\begin{table*}[ht]
\centering
\caption{End-to-End Latency, Latency of Compilation, Pure Inference Latency}
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{7}{c}{\textbf{Dataset}} \\ \cmidrule{3-9}
& & Citeseer&Cora&Pubmed&Flickr&Reddit&Yelp&ogbn-products\\ \midrule
\textbf{b1}&\begin{tabular}[|c|]{@{}c@{}}End-to-End latency $T_{\text{E2E}}$ (ms)\\latency of compilation $T_{\text{LoC}}$ (ms) \\Pure  inference latency  $T_{\text{PIL}}$ (ms)\end{tabular}
& \begin{tabular}[|c|]{@{}c@{}} 2.129 \\ 0.249 \\ 0.320 \end{tabular}  %%  Citeseer
& \begin{tabular}[|c|]{@{}c@{}} 0.808 \\ 0.215 \\ 0.103 \end{tabular}  %%  Cora
& \begin{tabular}[|c|]{@{}c@{}} 2.126 \\ 0.574 \\ 0.272 \end{tabular}  %%  Pubmed
& \begin{tabular}[|c|]{@{}c@{}} 9.97 \\ 2.68 \\ 1.28 \end{tabular}  %%  Flickr
& \begin{tabular}[|c|]{@{}c@{}} 128.3 \\ 51.1 \\ 15.6 \end{tabular}  %%  Reddit 
& \begin{tabular}[|c|]{@{}c@{}} 62.9 \\ 18.8 \\ 11.6 \end{tabular}  %%  Yelp
& \begin{tabular}[|c|]{@{}c@{}} 442 \\ 263.8 \\ 37.4 \end{tabular}  %%  ogbn-products 
\\ \midrule
\textbf{b2}&\begin{tabular}[|c|]{@{}c@{}}End-to-End latency $T_{\text{E2E}}$ (ms)\\latency of compilation $T_{\text{LoC}}$ (ms) \\Pure  inference latency  $T_{\text{PIL}}$ (ms)\end{tabular}
& \begin{tabular}[|c|]{@{}c@{}} 4.364\\ 0.254 \\ 2.55 \end{tabular}  %%  Citeseer
& \begin{tabular}[|c|]{@{}c@{}} 1.535 \\ 0.226 \\ 0.819 \end{tabular}  %%  Cora
& \begin{tabular}[|c|]{@{}c@{}} 4.28 \\ 0.66 \\ 2.34 \end{tabular}  %%  Pubmed
& \begin{tabular}[|c|]{@{}c@{}} 20.11 \\ 2.6 \\ 11.5 \end{tabular}  %%  Flickr
& \begin{tabular}[|c|]{@{}c@{}} 208.5 \\ 49.7 \\ 97.2 \end{tabular}  %%  Reddit 
& \begin{tabular}[|c|]{@{}c@{}} 155.1 \\ 18.3 \\ 104.3 \end{tabular}  %%  Yelp
& \begin{tabular}[|c|]{@{}c@{}} 718.1 \\ 261.4 \\ 315.9 \end{tabular}  %%  ogbn-products 
\\ \midrule
\textbf{b3}&\begin{tabular}[|c|]{@{}c@{}}End-to-End latency $T_{\text{E2E}}$ (ms)\\latency of compilation $T_{\text{LoC}}$ (ms) \\Pure  inference latency  $T_{\text{PIL}}$ (ms)\end{tabular}
& \begin{tabular}[|c|]{@{}c@{}} 4.355 \\ 0.235 \\ 2.56 \end{tabular}  %%  Citeseer
& \begin{tabular}[|c|]{@{}c@{}} 1.574  \\ 0.258 \\ 0.826 \end{tabular}  %%  Cora
& \begin{tabular}[|c|]{@{}c@{}} 4.25 \\ 0.59 \\ 2.38 \end{tabular}  %%  Pubmed
& \begin{tabular}[|c|]{@{}c@{}} 21.19 \\ 2.58 \\ 12.6 \end{tabular}  %%  Flickr
& \begin{tabular}[|c|]{@{}c@{}} 212.7 \\ 49.1 \\ 102.0 \end{tabular}  %%  Reddit 
& \begin{tabular}[|c|]{@{}c@{}} 134.3 \\ 19.2 \\ 82.6 \end{tabular}  %%  Yelp
& \begin{tabular}[|c|]{@{}c@{}} 657.4 \\ 272.2 \\ 244.4 \end{tabular}  %%  ogbn-products 
\\ \midrule
\textbf{b4}&\begin{tabular}[|c|]{@{}c@{}}End-to-End latency $T_{\text{E2E}}$ (ms)\\latency of compilation $T_{\text{LoC}}$ (ms) \\Pure  inference latency  $T_{\text{PIL}}$ (ms)\end{tabular}
& \begin{tabular}[|c|]{@{}c@{}} 6.912 \\ 0.212 \\ 5.14 \end{tabular}  %%  Citeseer
& \begin{tabular}[|c|]{@{}c@{}} 2.387 \\ 0.237 \\ 1.66 \end{tabular}  %%  Cora
& \begin{tabular}[|c|]{@{}c@{}} 6.919 \\ 0.599 \\ 5.04 \end{tabular}  %%  Pubmed
& \begin{tabular}[|c|]{@{}c@{}} 33.883 \\ 2.473 \\ 25.4 \end{tabular}  %%  Flickr
& \begin{tabular}[|c|]{@{}c@{}} 315 \\ 50.1 \\ 203.3 \end{tabular}  %%  Reddit 
& \begin{tabular}[|c|]{@{}c@{}} 278.2 \\ 21.3 \\ 224.4 \end{tabular}  %%  Yelp
& \begin{tabular}[|c|]{@{}c@{}} 905.2 \\ 270.3 \\ 494.1 \end{tabular}  %%  ogbn-products 
\\ \midrule
\textbf{b5}&\begin{tabular}[|c|]{@{}c@{}}End-to-End latency $T_{\text{E2E}}$ (ms)\\latency of compilation $T_{\text{LoC}}$ (ms) \\Pure  inference latency  $T_{\text{PIL}}$ (ms)\end{tabular}
& \begin{tabular}[|c|]{@{}c@{}} 14.899 \\ 0.239 \\ 13.1 \end{tabular}  %%  Citeseer
& \begin{tabular}[|c|]{@{}c@{}} 9.232 \\ 0.232 \\ 8.51 \end{tabular}  %%  Cora
& \begin{tabular}[|c|]{@{}c@{}} 15.636 \\0.556 \\ 13.8 \end{tabular}  %%  Pubmed
& \begin{tabular}[|c|]{@{}c@{}} 91.734 \\ 2.524 \\ 83.2 \end{tabular}  %%  Flickr
& \begin{tabular}[|c|]{@{}c@{}} 527.6 \\ 50.9 \\ 415.1 \end{tabular}  %%  Reddit 
& \begin{tabular}[|c|]{@{}c@{}} 901.6 \\ 30.1 \\ 839 \end{tabular}  %%  Yelp
& \begin{tabular}[|c|]{@{}c@{}} 1415.5 \\ 300.3 \\ 974.4 \end{tabular}  %%  ogbn-products 
\\ \midrule
\textbf{b6}&\begin{tabular}[|c|]{@{}c@{}}End-to-End latency $T_{\text{E2E}}$ (ms)\\latency of compilation $T_{\text{LoC}}$ (ms) \\Pure  inference latency  $T_{\text{PIL}}$ (ms)\end{tabular}
& \begin{tabular}[|c|]{@{}c@{}} 3.139 \\ 0.249 \\ 1.33 \end{tabular}  %%  Citeseer
& \begin{tabular}[|c|]{@{}c@{}} 1.201 \\ 0.258 \\ 0.453 \end{tabular}  %%  Cora
& \begin{tabular}[|c|]{@{}c@{}} 3.24 \\ 0.58 \\ 1.38 \end{tabular}  %%  Pubmed
& \begin{tabular}[|c|]{@{}c@{}} 17.686 \\ 2.686 \\ 8.99 \end{tabular}  %%  Flickr
& \begin{tabular}[|c|]{@{}c@{}} 219.2  \\ 50 \\ 107.6 \end{tabular}  %%  Reddit 
& \begin{tabular}[|c|]{@{}c@{}} 123.1 \\ 18.7 \\ 71.9 \end{tabular}  %%  Yelp
& \begin{tabular}[|c|]{@{}c@{}} 680.9 \\ 270.9 \\ 269.2 \end{tabular}  %%  ogbn-products 
\\ \midrule
\textbf{b7}&\begin{tabular}[|c|]{@{}c@{}}End-to-End latency $T_{\text{E2E}}$ (ms)\\latency of compilation $T_{\text{LoC}}$ (ms) \\Pure  inference latency  $T_{\text{PIL}}$ (ms)\end{tabular}
& \begin{tabular}[|c|]{@{}c@{}} 2.252 \\ 0.223 \\ 0.469 \end{tabular}  %%  Citeseer
& \begin{tabular}[|c|]{@{}c@{}} 0.826 \\ 0.235 \\ 0.101 \end{tabular}  %%  Cora
& \begin{tabular}[|c|]{@{}c@{}} 2.285 \\ 0.594 \\ 0.411 \end{tabular}  %%  Pubmed
& \begin{tabular}[|c|]{@{}c@{}} 11.321 \\ 2.631 \\ 2.68\end{tabular}  %%  Flickr
& \begin{tabular}[|c|]{@{}c@{}} 368.8 \\ 53.8 \\ 253.4  \end{tabular}  %%  Reddit 
& \begin{tabular}[|c|]{@{}c@{}} 72.1 \\ 17.5 \\ 22.1 \end{tabular}  %%  Yelp
& \begin{tabular}[|c|]{@{}c@{}} 601.8 \\ 261.4 \\ 199.6 \end{tabular}  %%  ogbn-products 
\\ \midrule
\textbf{b8}&\begin{tabular}[|c|]{@{}c@{}}End-to-End latency $T_{\text{E2E}}$ (ms)\\latency of compilation $T_{\text{LoC}}$ (ms) \\Pure  inference latency  $T_{\text{PIL}}$ (ms)\end{tabular}
& \begin{tabular}[|c|]{@{}c@{}} 7.981 \\ 0.231 \\ 6.19 \end{tabular}  %%  Citeseer
& \begin{tabular}[|c|]{@{}c@{}} 3.247 \\ 0.237 \\ 2.52 \end{tabular}  %%  Cora
& \begin{tabular}[|c|]{@{}c@{}} 13.791 \\ 0.611 \\ 11.9 \end{tabular}  %%  Pubmed
& \begin{tabular}[|c|]{@{}c@{}} 67.646 \\ 2.736 \\ 58.9 \end{tabular}  %%  Flickr
& \begin{tabular}[|c|]{@{}c@{}} 537.8 \\ 52.2 \\ 424 \end{tabular}  %%  Reddit 
& \begin{tabular}[|c|]{@{}c@{}} 548.2 \\ 28.7 \\ 487 \end{tabular}  %%  Yelp
& \begin{tabular}[|c|]{@{}c@{}} 1749.3 \\ 283.5 \\ 1325 \end{tabular}  %%  ogbn-products 
\\ \bottomrule
\end{tabular}
\label{tab:measured-latency-gnepu}
\end{table*}
\end{scriptsize}

==> experiments/resources.tex <==
%% div DSP 0 LUT 2 FF 16
%% EXP DSP 7 LUT 706 FF 408
%% ADD DSP 2 LUT 191 FF 365

%% RELU DSP 2 LUT 65 FF 68


